MiLeNAS: Efficient Neural Architecture Search via Mixed-Level Reformulation

Many recently proposed methods for Neural Architecture Search (NAS) can be formulated as bilevel optimization. For efficient implementation, its solution requires approximations of second-order methods. In this paper, we demonstrate that gradient errors caused by such approximations lead to suboptimality, in the sense that the optimization procedure fails to converge to a (locally) optimal solution. To remedy this, this paper proposes \mldas, a mixed-level reformulation for NAS that can be optimized efficiently and reliably. It is shown that even when using a simple first-order method on the mixed-level formulation, \mldas\ can achieve a lower validation error for NAS problems. Consequently, architectures obtained by our method achieve consistently higher accuracies than those obtained from bilevel optimization. Moreover, \mldas\ proposes a framework beyond DARTS. It is upgraded via model size-based search and early stopping strategies to complete the search process in around 5 hours. Extensive experiments within the convolutional architecture search space validate the effectiveness of our approach.

==> body.tex <==
%%%%%%%%% BODY TEXT
% Review (Shen Li): 
% 1. Introduction:
% contribution: 
% 1. optimizer (algorithm)
% 2. Early stopping and Searching and Evaluation 
% 3. Discussion: NAS charististics (empirical study)

% 2. Method:
% 3) Algorithm: enhance description

% Experiments: 
% (1) Complementary Materials; 
% (2) Related Works: deep architecture and architecture search: https://arxiv.org/pdf/1709.01507.pdf
% (3) mixed-level的优势: 通过超参分析实验，来验证算法/方法的性质
% ablation study: scale on channel or depth in efficient net: 统计一下train val 那个收敛时间和 parameter size，看看不同网络本身的参数对收敛性和parameter size影响.
% Channel Number: 对3x3 和1x1？你设置一个scale，比如从
% 0.5-8， 
% 0.75-12
% 1-16
% 1.5-24
% 2-32

% Depth: 另外就是depth，如果有时间的话，现在网络结构由normal和reduction组成，你可以设置一个depth scale，对normal，比如
% 0.5 - 4
% 0.75 - 6
% 1 - 8
% 1.5 - 12
% 2 - 16 
% reduction是不变的，因为stage不改，只是改变normal个数
% Interpretation Section: 1. motivation and logical flow 2. what is spectrum? 3. What's number range? 

% Related Works

% Review: 
% 1. in the NAS context (not only in the single-level optimization scenario), a low value of the validation loss that is minimized during the NAS loop, does not necessarily correlate with the true objective: minimizing the validation/test error of discrete architectures. [4] shows that actually the test accuracy of the final architectures does not correlate with the one-shot validation accuracy, and empirically demonstrate that there is an overfitting on the architectural level.

% different hyperparameter settings compared to baselines in the final training of found architectures. Section 3.3: How did you tune the learning rate (0.03 vs 0.025 in DARTS)?

% just one run of their methods in some settings in Table 1 and in Table 2.

% What are the settings you use for your algorithm in Table 1?

% [Experiments] Experiments showing how the performance of the architectures found by bi-level optimization relates with the solution returned by the inner problem, i.e. the number of gradient steps towards the approximated w^*.

% [method] What is the difference between the proposed method and the first-order variant of DARTS? Why does the proposed MiLeNAS yield better results than the first-order variant of DARTS? Why does MiLeNAS (0.3 GPU day) take less training cost than the first-order variant of DARTS (1.5 GPU day)? More explanations are required.

% [Introduction + Method] The authors argue that DARTS fails to converge to an optimal solution since the optimal w*(alpha) cannot be obtained via a single step training. However, MiLeNAS also uses the same single step training technique. Thus, this issue also occurs in the proposed MiLeNAS method


% [method, experiment] What would happen if the proposed MiLeNAS method uses the second-order approximation?

% [Experiment] The results in Figure 3 are not convincing. For example, bilevel (1st) method achieves higher accuracy than bilevel (2nd) method, which conflicts with results in DARTS[1]. More discussions on this phenomenon are required.

% [Experiment] Some experiment results are very confusing. In Table 1, the authors provide four results of MiLeNAS but do not mention the differences among them. The similar issue also exists in Table 2.

% [Experiment] In Section 3.3, the authors mention that the proposed method can further improve XNAS[2]. However, there are no experiments to verify this argument.

% [Experiment] Several state-of-the-art NAS methods should be compared in the experiments, such as PROXYLESSNAS[3] and P-DARTS[4].

% [Introduction] The authors mention that “evolutionary algorithms and reinforcement learning-based methods require thousands of GPU days to achieve state-of-the-art performance”. However, this argument is wrong. In fact, ENAS is a typical reinforcement learning-based method and only takes 0.5 GPU days to train the model.

% [Introduction] In the third paragraph of Page 2, “gap between the training loss and the evaluation loss” should be “gap between the training accuracy and the evaluation accuracy”.

% [Method] The structure of this paper can be improved. The main content of Section 2.3 is to describe how to demonstrate the effectiveness of the proposed method, which is more relevant to Section 3. Therefore, it is better to put Section 2.3 in Section 3.

% [Experiment] In Figure 2, the caption should be put below the graphic.

% [method] However, reformulating Eq. (1)(2) to Eq. (4) is incremental and completely not new in the optimization field.

% [Abstract] It says that "The existing second order failed to converge to a optimal solution but the proposed method can be optimized more reliably". There is no evidence to support this, neither theoretically or empirically. In the results, the proposed approximation obtained comparable results as the second order approximation method DARTS, e.g. in Table 1.

% [Novelty] It also claimed that both single and bilevel optimization are special case of the proposed method. This is not correct. The proposed method is more like approximation solver for the bilevel optimization problem.

%----------------------
% \section{\textcolor{red}{Structure Reorganization}}
% Motivation: Gradient-based methods (DARTS, GDAS) has attracted a lot of attention due to its simplicity and small search costs achieved by a continuous relaxation and an approximation of the resulting bi-level optimization problem. 
% However, according to our investigation, there several problems in such method:

% 1. The second order approximation has gradient-error, a faster and robust optimization method is needed.

% 2. The gradient-based searching algorithm is a block-box to architecture design, which does not provide any insight to searching strategy and design choice for CNN architecture. Specially, through tracking the parameter size during the search process, we found the original DARTS will decrease its parameter size in the later phase of the searching period. 

% To address these problems, we proposed MiLeNAS: an algorithm and framework to run on different search spaces, optimization methods, multi-parameter size tracking, early stopping strategy, and parameter size evaluation.

% MiLeNAS has two significant benefits:

% 1. reformulate the bi-level optimization NAS as a mixed-level optimization, leading to higher accuracy while enjoying faster searching speed.

% 2. reliable
% 2. Through tracking the parameter size during the search process, we found MiLeNAS has as a distinct phase-by-phase optimization characteristic in the search process. This provides three major insights for neural architecture design: (1) for a specific learning task, the most economical neural network architecture must be identified, and the redundant parameter quantity cannot bring additional benefits. (2) our method has the potential to be an alternative method for model  compression  since  it  can  find  multiple  optimal  architectures under different computational complexities. (3) Most importantly, we may figure out a regular pattern between the parameter number and the architecture accuracy, allowing us to further refine a strategy to speed the search process. In our case, we have found that the early stopping strategy can remarkably increase the search speed. 

% Remark: our experiment in DARTS does not consistently show the same characteristics as in MiLeNAS. We argue that this regular pattern from the observation is attributed to the rubustness of our mixed-level optimization since we correlate the relationship between the validation and evaluation dataset for updating $\alpha$.

\section{\textcolor{red}{Structure Reorganization}}
Motivation: Gradient-based methods (DARTS, GDAS) has attracted a lot of attention due to its simplicity and small search costs achieved by a continuous relaxation and an approximation of the resulting bi-level optimization problem. 
However, according to our investigation, there several problems in such method:

1. The second order approximation has gradient-error, a faster and robust optimization method is needed.

2. The gradient-based searching algorithm is a block-box to architecture design, which does not provide any insight to searching strategy and design choice for CNN architecture. Specially, through tracking the parameter size during the search process, we found the original DARTS will decrease its parameter size in the later phase of the searching period. 

To address these problems, we proposed MiLeNAS: an algorithm and framework to run on different search spaces, optimization methods, multi-parameter size tracking, early stopping strategy, and parameter size evaluation.

MiLeNAS has two significant benefits:

1. reformulate the bi-level optimization NAS as a mixed-level optimization, leading to higher accuracy while enjoying faster searching speed.

2. Through tracking the parameter size during the search process, we found MiLeNAS has as a distinct phase-by-phase optimization characteristic in the search process. This provides three major insights for neural architecture design: (1) for a specific learning task, the most economical neural network architecture must be identified, and the redundant parameter quantity cannot bring additional benefits. (2) our method has the potential to be an alternative method for model  compression  since  it  can  find  multiple  optimal  architectures under different computational complexities. (3) Most importantly, we may figure out a regular pattern between the parameter number and the architecture accuracy, allowing us to further refine a strategy to speed the search process. In our case, we have found that the early stopping strategy can remarkably increase the search speed. 

Remark: our experiment in DARTS does not consistently show the same characteristics as in MiLeNAS. We argue that this regular pattern from the observation is attributed to the rubustness of our mixed-level optimization since we correlate the relationship between the validation and evaluation dataset for updating $\alpha$.
